Determinacy from strong compactness of $\omega_1$

In the absence of the Axiom of Choice, the "small" cardinal $\omega_1$ can exhibit properties more usually associated with large cardinals, such as strong compactness and supercompactness. For a local version of strong compactness, we say that $\omega_1$ is $X$-strongly compact (where $X$ is any set) if there is a fine, countably complete measure on $\mathcal{P}_{\omega_1}(X)$. Working in $\mathsf{ZF} + \mathsf{DC}$, we prove that the $\mathcal{P}(\omega_1)$-strong compactness and $\mathcal{P}(\mathbb{R})$-strong compactness of $\omega_1$ are equiconsistent with $\mathsf{AD}$ and $\mathsf{AD}_\mathbb{R} + \mathsf{DC}$ respectively, where $\mathsf{AD}$ denotes the Axiom of Determinacy and $\mathsf{AD}_\mathbb{R}$ denotes the Axiom of Real Determinacy. The $\mathcal{P}(\mathbb{R})$-supercompactness of $\omega_1$ is shown to be slightly stronger than $\mathsf{AD}_\mathbb{R} + \mathsf{DC}$, but its consistency strength is not computed precisely. An equiconsistency result at the level of $\mathsf{AD}_\mathbb{R}$ without $\mathsf{DC}$ is also obtained.

==> ADRDC.tex <==
\section{$\sf{AD}_\mathbb{R}$ AND $\sf{AD}_\mathbb{R} + \sf{DC}$}
We continue with the proof of Theorem \ref{lowerbound}. In the previous section, we have shown that the Solovay sequence of $\Omega$ cannot have successor length, in other words, it cannot be the case that $\Omega = \powerset(\mathbb{R})\cap \Lp^{^\gTheta\F}(\mathbb{R},\F\rest\mathbb{R})$ for some operator $\F$ since otherwise, we can then construct a suitable operator $\mathcal{G}$ such that $\mathcal{G}\rest\mathbb{R}\notin \Omega$ and $\Lp^{^\gTheta\mathcal{G}}(\mathbb{R},\mathcal{G}\rest\mathbb{R})\vDash \textsf{AD}$. This contradicts the definition of $\Omega$.

Recall from Section \ref{omega_closed} the following:
\begin{itemize}
\item $L[\mathcal{H}](\Omega)$ is a symmetric extension of $L[\mathcal{H}]$ via $\mathbb{P}$.
\item $\powerset(\mathbb{R})\cap L[\mathcal{H}](\Omega) = \Omega$; so $L[\mathcal{H}](\Omega)\vDash \sf{AD}_\mathbb{R}$
\end{itemize}
Lemma \ref{NotProjecting} shows that $V_{\Theta^\Omega}\cap L[\mathcal{H}] = |\mathcal{H}|$. In the case $L[\mathcal{H}] \vDash$ ``there are $\omega$ many Woodin cardinals", let $M$ be the derived model of $L[\mathcal{H}]$ (at the supremum of $L[\mathcal{H}]$'s Woodin cardinals). Then $M\vDash \sf{AD}_\mathbb{R}$ (cf. \cite[Section 3.3]{ATHM}). This would be enough to complete the proof of Theorem \ref{ADREqui}, but Section \ref{omega_closed} proves something stronger, namely, $\Omega$ is constructibly closed. 
\begin{lemma}\label{ADRDC}
If $\sf{DC}$ holds, then cof$(\Theta^\Omega)>\omega$ and $L[\mathcal{H}](\Omega) \vDash \sf{AD}_\mathbb{R} + \sf{DC}$.
\end{lemma}
\begin{proof}
Suppose cof$(\Theta^\Omega) = \omega$. Let $M$ be a transitive structure containing $\mathcal{H}^+\cup \Omega$, where $\mathcal{H}^+=L[\mathcal{H}]|\gamma$, where $\gamma>\Theta^\Omega$ is a regular cardinal in $L[\mathcal{H}]$. Let $\sigma\prec M$ be countable such that $\sigma$ is cofinal in $\Theta^\Omega$. Now the $\pi_\sigma$-realizable strategy $\Sigma_\sigma$ defined in the proof of Lemma \ref{NotProjecting} acts on $\pi^{-1}_\sigma(\mathcal{H}^+)$. $\Sigma_\sigma$ on stacks below $\Theta_\sigma$ is simply $\Sigma_\sigma^-$ in this case; by replacing $(\N_\sigma,\Sigma_\sigma)$ by an iterate, we may assume $\Sigma_\sigma$ has branch condensation. We can show then that $\Sigma_\sigma\in \Omega$ as before. Furthermore, letting $i$ be the direct limit map from $\pi_\sigma^{-1}(\mathcal{H}^+)$ into the direct limit $\M_\infty$ of all of its $\Sigma_\sigma$-iterates in $\Omega$, then by elementarity
\begin{center}
$\pi_\sigma \rest \Theta_\sigma = i\rest \Theta_\sigma$.
\end{center}
So $i$ is cofinal in $\Theta^\Omega$. This means $\M_\infty|\delta^{\M_\infty} = \mathcal{H}\notin \Omega$. But this contradicts the fact that $\Sigma_\sigma\in \Omega$.

The second clause follows immediately from the first and the remarks above.

\end{proof}

Lemma \ref{ADRDC} completes the proof of the following theorems.
\begin{theorem}[$\sf{ZF+DC}_\mathbb{R}$]\label{ADR}
Suppose $\Omega=\{A\subseteq \mathbb{R} \ | \ L(A,\mathbb{R})\vDash \sf{AD}^+\}$ and $(\dag)$ holds. Suppose $\Omega\neq \emptyset$ and for every suitable pair $(\P,\Sigma)$ or hod pair $(\P,\Sigma)$ such that $\Sigma$ has branch condensation and is $\Omega$-fullness preserving, $\Sigma\in \Omega$. If the Solovay sequence of $\Omega$ has limit length, then there is a $\Gamma \unlhd_w \Omega$ such that $\Gamma = L(\Gamma,\mathbb{R})\cap \powerset(\mathbb{R})$ and $L(\Gamma,\mathbb{R})\vDash \sf{AD}_\mathbb{R}$.
\end{theorem}
\begin{theorem}[$\sf{ZF+DC}$]\label{ADR+DC}
Suppose $\Omega=\{A\subseteq \mathbb{R} \ | \ L(A,\mathbb{R})\vDash \sf{AD}^+\}$ and $(\dag)$ holds. Suppose $\Omega\neq\emptyset$ and for every suitable pair $(\P,\Sigma)$ or hod pair $(\P,\Sigma)$ such that $\Sigma$ has branch condensation and is $\Omega$-fullness preserving, $\Sigma\in \Omega$. If the Solovay sequence of $\Omega$ has limit length, then $L(\Omega,\mathbb{R})\cap \powerset(\mathbb{R})=\Omega$ and $L(\Omega,\mathbb{R})\vDash \sf{AD}_\mathbb{R} + \sf{DC}$.
\end{theorem}

Lemma \ref{NextTheta} and Theorems \ref{ADR}, \ref{ADR+DC} complete the proof of Theorems \ref{ADREqui}, \ref{lowerbound}, and \ref{equiconsistency}. 



==> Scales.tex <==
\section{Scales analysis in $K^\Sigma(\mathbb{R})$}
Assume $\Sigma$ is a strategy for a mouse with branch condensation. Our official definition of $K^\Sigma(\mathbb{R})$ can be found in \cite{ATHM}. In general the scale analysis is independent of specific definitions of $K^\Sigma(\mathbb{R})$. The important thing to note is that if $\M\lhd K^\Sigma(\mathbb{R})$ then the levels of $\M$ that we add branches for a tree according to $\Sigma$ are $ZF$ models. The language $\mathcal{L}$ for $\Sigma$-premice over $\mathbb{R}$ is just $\mathcal{L}^* \cup \{S,b\}$ where $\mathcal{L}^*$ is the language for $\mathbb{R}$-premice used in \cite{K(R)} and $S$ is a binary predicate whose intended interpretation is some strategy (in this case, a part of the strategy for $\M_1^{\Sigma,\sharp}$) and $b$ is the predicate for the branch of a tree according to $S$. So $\M$ can be active because either $\dot{F} \neq \emptyset$ or $b\neq \emptyset$.
\\
\indent We'll use the $\H_\Sigma$ analysis outlined in the next subsection section and game theoretic techniques to prove 
\begin{theorem}
\label{passive game scale}
Suppose $\M$ is a passive, countably iterable $\Sigma$-premouse over $\mathbb{R}^\M$ and suppose $\M \vDash \rm{AD}$. Then $\M \vDash \textrm{``the pointclass } \undertilde{\Sigma}^\M_1 \textrm{ has the scale property."}$
\end{theorem} 

\begin{definition}
\label{sigma 1 elem}
Let $\M$ and $\N$ be $\Sigma$-premice over some set $X$ (here we don't assume $\M$ and $\N$ satisfy choice). We write $\M \prec_1 \N$ iff $\M$ is an initial segment of $\N$ and whenever $\psi(v_1,...,v_n)$ is a $\Sigma_1$ formula of the language $\mathcal{L}$ in which $\dot{F}, \dot{\mu}, \dot{\nu},$ and $\dot{\gamma}$ do not occur then for any $a_1,...,a_n \in X \cup \{X\}$,
\begin{equation*}
\N \vDash \psi[a_1,...,a_n] \Rightarrow \M \vDash \psi[a_1,...,a_n].
\end{equation*}
\end{definition}
Note that in the above definition, $\psi$ can mention $S$ but not $b$ since $\N$ does not satisfy $ZF$.
\begin{definition}
\label{gap}
Let $\M$ be a $\Sigma$-premouse over some set $X$ and suppose $\omega\alpha \leq \omega\beta \leq o(\M)$. We call the interval $[\alpha,\beta]$ a $\Sigma_1$-gap of $\M$ iff
\begin{enumerate}
\item $\M|\alpha \prec_1 \M|\beta$,
\item $\forall \gamma < \alpha (\M|\gamma \nprec_1 \M|\alpha)$,
\item $\forall \gamma > \beta  (\M|\beta \nprec_1 \M|\gamma)$.
\end{enumerate}
\end{definition}
\begin{theorem}\label{BeginGap}
Let $\M$ be a countably $0$-iterable $\Sigma$-mouse over $\mathbb{R}^\M$. Let $\alpha$ begin a gap in $\M$ and $\M|\alpha \vDash \rm{AD}$; then $\M$ believes that the pointclass $\undertilde{\Sigma}_1^{\M|\alpha}$ has the scale property.
\end{theorem}
%We define strong and weak gaps just as in \cite{ScalesK(R)} but here types are in the language $\mathcal{L}$. Here are the two main theorems regarding the scale pattern at the end of gaps.

%\begin{theorem}
%\label{strong gap}
%Let $\M$ be a countably 0-iterable $\Sigma$-mouse over $\mathbb{R}^\M$ which satisfies AD. Let $[\alpha,\beta]$ be a strong $\Sigma_1$-gap of $\M$ such that $\omega\beta < o(\M)$; then
%\begin{enumerate}[(a)]
%\item there is a $\Pi_1^{\M|\alpha}$ relation on $\mathbb{R}^\M$ which has no uniformization which is definable over $\M|\beta$, and hence
%\item $\M$ believes that none of the pointclasses $\Sigma_n^{\M|\beta}$ or $\Pi_n^{\M|\beta}$ have the scale property.
%\end{enumerate}
%\end{theorem}
%\indent Hence, at the end of strong gaps $[\alpha,\beta]$, the scale property first reappers with the pointclass $\Sigma_1^{\M|(\beta+1)}$. For the weak gap case, we prove the analogue of Theorem 0.1 in \cite{Scalesweakgap}.
%\begin{theorem}
%\label{weak gap}
%Let $\M$ be a countably $\omega$-iterable $\Sigma$-mouse over $\mathbb{R}^\M$ which satisfies AD and $[\alpha, \beta]$ is a weak gap of $\M$ $(\beta$ may be $o(\M))$. Suppose $\Gamma =_{def} \Sigma_1^{\M|\alpha}$ is captured by mice with iteration strateies in $\M|\alpha$, ie., $\forall b \in HC^\M (Lp^{\Sigma,\Gamma}(b)\cap \powerset(b) = C_\Gamma(b))$. Then we have that $\M$ believes that $\Sigma_n^{\M|\beta}$ has the scale property where $n$ is least such that $\rho_n(\M|\beta) = \mathbb{R}^\M$.  
%\end{theorem}
The proof of Theorem \ref{BeginGap} follows from that of Theorem \ref{passive game scale}. The pattern of scales at the end of gaps is analyzed in the second author's thesis \cite{wilson2012contributions}. This work is particularly useful in the core model induction arguments in this paper.
\subsection{Local $HOD_\Sigma$ analysis}
Let $\M$ be a $\Sigma$-premouse over $\mathbb{R}^\M$ and $\M \vDash ``\Theta$ exists." Set $\theta = \Theta^\M$. Fix an $n_0$ such that $\M$ is $n_0$-sound and $\rho_{n_0}(\M) \geq \theta$. Letting $o(\M) = \omega\gamma_0$, we assume that for all $\langle \xi, k\rangle <_{lex} \langle \gamma_0,n_0\rangle$, $\M|\xi$ is countably $k$-iterable. Finally, let 
\begin{equation*}
T^\M = \{\langle \phi, \vec{\alpha}\rangle \ | \ \phi \in \mathcal{L}, \ \vec{\alpha}\in ^{<\omega}\theta \textrm{ and } \M|\theta \vDash \phi[\vec{\alpha}] \}.
\end{equation*}
\indent We define $\mathcal{H}$: a $\Sigma$-premouse over $T^\M$  by the same process as that in \cite{ScalesK(R)}. Namely starting at a least $\lambda$ such that $\M|\lambda \vDash ZF$, we let
\begin{equation*}
\mathcal{H}_\alpha = \mathcal{J}_\alpha(\theta \cup \{T^\M\}).
\end{equation*} 
We then do a level-by-level translation of extenders from $\M$ to that of $\mathcal{H}$ and literally feed in the same trees to the $\mathcal{H}$ side from the corresponding levels on the $\M$ side. That this can be done is implicit in the definition of a $\Sigma$-premouse over $\mathbb{R}$.
\\
\indent Working in $\M$, we define the Vopenka algebra $Vop_\omega$ that adds an enumeration of $\mathbb{R}^\M$ to $\mathcal{H}$ as in \cite{ScalesK(R)} but definitions can mention the predicate for the strategy. It's easy to see that $Vop_\omega \in \mathcal{H}_2$. Truth in $\mathcal{H}(\mathbb{R}^\M)$ can be reduced to truth in $\mathcal{H}$ via the forcing relation for $Vop_\omega$. Also $\mathcal{H}(\mathbb{R}^\M)$ determines $\M$ by the local definability of the forcing. The local definability of the forcing is also used to show that the reduction of $\M$-truth to $\mathcal{H}$-truth is local. The following is the main theorem, whose proof is just that in \cite{ScalesK(R)}.
\begin{theorem}
\label{local def}
$\mathcal{H}$ is a $\Sigma$-premouse over $T^\M$; moreover, for all $k\leq n_0$, $\mathcal{H}$ is $k$-sound, $\rho_k(\mathcal{H}) = \rho_k(\mathcal{M})$, and $p_k(\mathcal{H}) = p_k(\mathcal{M})\backslash \{\theta\}$.
\end{theorem}
\indent From the proof of Theorem \ref{local def}, we see that if $\M \vDash ZF^-$ then
\begin{equation*}
x \in \mathcal{H} \Leftrightarrow \exists \alpha(\omega\alpha < \omega\gamma_0 \wedge \forall y \in tcl(x)\cup\{x\}(y \in OD^{\M|\alpha}_\Sigma)).
\end{equation*}
So $\mathcal{H}$ indeed carries the intended meaning for $HOD_\Sigma^\M$. The next theorem relates the iterability of $\mathcal{H}$ and $\M$. It is the reason we isolate $\mathcal{H}$, which is an important ingredient in our proof of Theorem \ref{passive game scale}.
\begin{theorem}
Let $\M$ be $n_0$-sound $\Sigma$-premouse over $\mathbb{R}^\M$ and $\M \vDash ``\Theta$ exists." Suppose $\rho_{n_0}(\M) \geq \Theta^\M$ and $\M|\lambda \vDash ZF$ for some $\lambda \geq \Theta^\M$. Suppose $\M|\xi$ is countably $k$-iterable for all $\langle \xi, k\rangle <_{lex} \langle \gamma_0,n_0\rangle$ such that $\xi \geq \Theta^\M$ and $\omega\gamma_0 = o(\M)$. Let $\mathcal{H}$ be defined in $\M$ as above. Then for all $\gamma$,
\begin{equation*}
\mathcal{H} \textrm{ is } (n_0,\gamma)\textrm{-iterable} \Rightarrow \M \textrm{ is } (n_0,\gamma)\textrm{-iterable above }\Theta^\M.
\end{equation*}
\end{theorem}
\subsection{The scale property in $K^\Sigma(\mathbb{R})$}
\textit{Proof sketch of Theorem \ref{passive game scale}.} Fix a countable passive, coutably 0-iterable $\mathbb{R}^\M$-premouse $\M$. Assume also $\M \vDash \rm{AD}$ and $o(\M) = \omega\alpha$ where $\alpha$ is a limit ordinal. The case where $\alpha$ is successor is handled by ideas similar to that of the limit case and by considering the $\S$ hierrarchy. See \cite{Scales} for details.
\\
\indent Let $\phi_0$ be a $\Sigma_1$ formula in the language $\mathcal{L}$ where we may assume (by the fact that $\M$ is passive) that the constants $\dot{F}, \dot{\mu}, \dot{\nu}, \dot{\gamma}$ for the top extender don't occur in $\phi_0$. Hence $\phi_0$ can only mention $\dot{\in}, \dot{E}, \dot{\mathbb{R}}, S$. For $x \in \mathbb{R}^\M$, let
\begin{equation*}
P(x) \Leftrightarrow \M \vDash \phi_0[x].
\end{equation*} 
We show that $\M$ thinks there is a $\Sigma^\M_1$-scale on $P$.
\\
\indent First let $\alpha^* = \Theta^\M$ if $\M \vDash \Theta$ exists; otherwise, let $\alpha^* = o(\M)$. Then $\P = \displaystyle \cup_{\beta<\alpha^*} P^\beta$ where for $x \in \mathbb{R}^\M$,
\begin{equation*}
P^\beta(x) \Leftrightarrow \M|\beta \vDash \phi_0[x].
\end{equation*}
For each $\beta<\alpha^*$, we construct a closed game representation $x \mapsto G^{\beta}_x$ for $P^\beta$ where $G^\beta_x$ is a closed game defined below that is continuously associated to $x$. Let 
\begin{eqnarray*}
P^\beta_k(x,u) &\Leftrightarrow& u\textrm{ is a position of length } k \textrm{ from which player I has a winning} \\&& \textrm{quasi-strategy in } G^\beta_x. 
\end{eqnarray*}
We will define $G^\beta_x$ in such a way that $P^\beta_k \in \M$ and the map $\langle\beta,k\rangle \mapsto P^\beta_k$ is $\Sigma_1^\M$. This will give us the desired $\Sigma_1^\M$ scale.
\\
\indent Fix $\beta<\alpha^*$ and $x \in \mathbb{R}^\M$. We want to define $G^\beta_x$. The idea of the game is as follows. Player I plays a countable model of ``$V = K^\Sigma(\mathbb{R}) + \phi_0(x) + \forall \gamma \ \mathcal{J}^{\vec{E},\Sigma}_\gamma(\mathbb{R})\nvDash \phi_0[x]$" that contains all reals played by player II. Player I also needs to verify second order facts about his model to prove that he is playing an $\N$ that is an $\mathbb{R}^\N$-mouse. Wellfoundedness of $\N$ is verified by embedding $\N$'s ordinals into $\omega\beta$ and iterability of $\N$ is verified by embedding the local $HOD_\Sigma$'s of $\N$ into the corresponding local $HOD_\Sigma$'s of $\M|\beta$ under his embedding of ordinals.
\\
\indent The language for the game is that of $\mathcal{L}^* =_{\textrm{def}} \mathcal{L} \cup \{\dot{x_i} \ | \ i <\omega\} \cup \{\dot{a}\}$ where the constant symbols $\dot{x_i}$ will denote the $i^{th}$ real played in the game and $\dot{a}$ will denote $\M_1^{\Sigma,\sharp}$. Fix recursive maps
\begin{equation*}
m,n: \{\ulcorner\sigma\urcorner \ | \ \sigma \textrm{ is an } \mathcal{L^*}-\textrm{formula}\} \rightarrow \{2n \ | \ 1 \leq n < \omega\}
\end{equation*}
which are one-to-one, have disjoint recursive ranges, and are such that whenever $\dot{x_i}$ occurs in $\sigma$, then $i <  \min(m(\sigma),n(\sigma))$. For an $\mathbb{R}^\P$-premouse $\P$ and $\xi < o(\N)$, $\P \vDash \xi$ is relevant iff $\P|\xi \vDash ``\Theta$ exists, and there is a $\lambda > \Theta$ such that $\mathcal{J}^{\dot{E},\Sigma}_{\lambda}\vDash \rm{ZF}$".
\\
\indent Fix a $\Sigma_1$ formula $\sigma_0(v_0,v_1,v_2)$ that uniformly defines the graph of a surjection $h_\gamma: [\omega\gamma]^{<\gamma}\times\mathbb{R} \twoheadrightarrow \M|\gamma$ over $\M|\gamma$ for each $\gamma$. Let $T$ be the following $\mathcal{L}^*$ theory
\\
\indent\indent $(1)$ \ \ \ Extensionality + $V = K^\Sigma(\mathbb{R})$\\
\indent\indent $(2)$ \ \ \ $\forall v (v \textrm{ is relevant} \Rightarrow \mathcal{H}_v \textrm{ exists})$\\
\indent\indent $(3)_{\phi}$ \ \ $\exists v\phi(v) \Rightarrow \exists v (\phi(v)\wedge \forall u\in v \neg \phi(u))$ \\
\indent\indent $(4)_i$ \ \ $\dot{x_i} \in \mathbb{R}$\\
\indent\indent $(5)$ \ \ \ $\phi_0(\dot{x_0}) \wedge \forall \gamma(\mathcal{J}^{\dot{E},\Sigma}_\gamma(\mathbb{R})\nvDash \phi_0[\dot{x_0}])$\\
\indent\indent $(6)$ \ \ \ $\forall v_0,v_1,y,z(\sigma_0(v_0,v_1,y)\wedge \phi_0(v_0,v_1,z) \Rightarrow y = z)$ \\
\indent\indent $(7)_{\phi}$ \ \ $\exists v \phi(v) \Rightarrow \exists v\exists F\in [Ord]^{<\omega}(\phi(v) \wedge \sigma_0(F,\dot{x}_{m(\ulcorner\phi\urcorner)},v))$\\
\indent\indent $(8)_\phi$ \ \ $\exists v(\phi(v) \wedge v\in\mathbb{R}) \Rightarrow \phi(\dot{x}_{n(\ulcorner\phi\urcorner)})$.\\
\indent A run of the game $G^\beta_x$ is of length $\omega$. For each $n$, player I plays $i_n,x_{2n},\eta_n$ where $i_n \in \{0,1\}$, $x_{2n} \in \mathbb{R}$, and $\eta_n < \omega\beta$ while player II plays $x_{2n+1} \in \mathbb{R}$. If $u = \langle(i_k,x_{2k},\eta_k,x_{2k+1}) \ | \ k < n\rangle$ is a partial play of length $n$, we let
\begin{equation*}
T^*(u) = \{\sigma \ | \ \sigma \textrm{ is a sentence of } \mathcal{L}^* \wedge i_{n(\ulcorner\sigma\urcorner)} = 0 \wedge n(\sigma) < n\},
\end{equation*}
and if $p$ is a full run of $G^\beta_x$,
\begin{equation*}
T^*(p) = \bigcup_{n<\omega}T^*(p\rest n).
\end{equation*}
For notational convenience, we let ``$iv\phi(v)$" stand for ``the least $v$ such that $\phi(v)$". $p = \langle(i_k,x_{2k},\eta_k,x_{2k+1}) \ | \ k < \omega\rangle$ is a winning run for player I iff
\begin{enumerate}[(a)]
\item $x_0 = (x, \M_1^{\Sigma,\sharp})$,
\item $T^*(p)$ is a complete consistent extension of $T$ and for all $i,m,n<\omega$, $``\dot{x}_i(n) = m" \in T^*(p)$ iff $x_i(n) = m$,
\item ``$\varphi \in \dot{a}$"$\in T^*(p)$ iff $\varphi \in \M_1^{\Sigma,\sharp}$,
\item if $\phi$ and $\psi$ are $\mathcal{L}^*$-formulae with one free variable and ``$iv\phi(v) \in \textrm{Ord} \wedge iv\psi(v) \in \textrm{Ord}$"$\in T^*(p)$, then ``$iv\phi(v) \leq iv\psi(v)$"$\in T^*(p)$ iff $\eta_{n(\ulcorner\phi\urcorner)} \leq \eta_{n(\ulcorner\psi\urcorner)}$,
\item if $\psi$ is an $\mathcal{L}^*$-formula with one free variable and ``$iv\psi(v) \in \textrm{Ord} \wedge iv\psi(v) \textrm{ is relevant}$"$\in T^*(p)$, then $\eta_{n(\ulcorner\psi\urcorner)}$ is relevant in $\M$. Furthermore, if $\sigma_1,\dots, \sigma_n$ are $\mathcal{L}^*$-formulae of one free variable such that for all $k$, ``$iv\sigma_k(v) < iv\psi(v)$"$\in T^*(p)$ then for any $\mathcal{L}$-formula $\theta(v_1,\dots,v_n)$,
\begin{equation*}
``\mathcal{H}_{iv\psi(v)}\vDash \theta[iv\sigma_1(v),\dots,iv\sigma_n(v)]"\in T^*(p)
\end{equation*}
if and only if
\begin{equation*}
\mathcal{H}^\M_{\eta_{n(\ulcorner\psi\urcorner)}}\vDash \theta[\eta_{n(\ulcorner\sigma_1\urcorner)},\dots,\eta_{n(\ulcorner\sigma_n\urcorner)}].
\end{equation*}
\end{enumerate}
We now define the notion of \textit{honesty} and show that player I wins if and only if he is honest. More precisely, we say a position $u = \langle(i_k,x_{2k},\eta_k,x_{2k+1}) \ | \ k < n\rangle$ is $(\beta,x)$-\textbf{honest} iff $\M|\beta \vDash \phi_0[x]$ and letting $\gamma\leq \beta$ be the least such that $\M|\gamma\vDash \phi_0[x]$, we have
\begin{enumerate}[(i)]
\item $n>0 \Rightarrow x_0 = (x,\M_1^{\Sigma,\sharp})$,
\item if we interpret $\dot{x}_i$ as $x_i$ for $0 < i < 2n$ and $(\dot{x_0},\dot{a})$ as $x_0$ then all axioms of $T^*(u)\cup T$ as interpreted in $(\M|\gamma,I_u)$ are true there where $I_u$ is the aforementioned interpretation, and
\item if $\sigma_0,\dots,\sigma_m$ enumerate $\mathcal{L}^*$-formulae $\sigma$ of one free variable such that $n(\ulcorner\sigma\urcorner) < n$ and 
\begin{equation*}
(\M|\gamma,I_u) \vDash iv\sigma(v) \in \textrm{Ord},
\end{equation*}
and if $\delta_i < \omega\gamma$ such that
\begin{equation*}
(\M|\gamma,I_u) \vDash iv\sigma(v) = \delta_i,
\end{equation*}
then the map
\begin{equation*}
\delta_i \mapsto \eta_{n(\ulcorner\sigma_i\urcorner)}
\end{equation*}
is well-defined and extendible to an order preserving map $\pi:\omega\gamma \rightarrow \omega\beta$ such that whenever $\delta_i$ is relevent in $\M$ then $\pi|\omega\delta_i$ is extendible to an elementary embedding from $\mathcal{H}^\M_{\delta_i}$ to $\mathcal{H}^\M_{\eta_{n(\ulcorner\sigma_i\urcorner)}}$. Here we note that elements in $\mathcal{H}^\M_{\delta_i}$ are definable from ordinals in $\omega\delta_i$ since our language involves the predicate $S$ for the strategy of $\M_1^{\Sigma,\sharp}$.
\end{enumerate}
The following two claims complete our proof of theorem 1.1. The proof of these claims is similar to that of claims 4.2, 4.3 in \cite{ScalesK(R)}.
\\
\\
\indent \textit{Claim 1.} Letting $Q^\beta_k(x,u)$ iff $u$ is a $(\beta,x)$-honest position of length $k$, we have that $Q^\beta_k \in \M$ for all $\beta$, and the map $(\beta,k)\mapsto Q^\beta_k$ is $\Sigma_1^\M$.
\\
\\
\indent \textit{Claim 2.} For any position $u$ in $G^\beta_x$, player I has a winning quasi-strategy starting from $u$ iff $u$ is $(\beta,x)$-honest, i.e., $P^\beta_k(x,u) \Leftrightarrow Q^\beta_k(x,u)$ for all $k$.
%\indent We now move on to the proof of Theorem \ref{strong gap}. We give a proof using mouse capturing because it's not clear to us that Martin's reflection theorem (for the inductive pointclass) obviously generalizes to other inductive-like pointclasses (like $\Sigma_1$ of the strong gap). A careful look at the proof shows that it actually implies Martin's reflection theorem in our situation. Theorem \ref{strong gap} combined with Theorem \ref{passive game scale} imply that the scale pattern first reappears at the pointclass $\Sigma_1^{\M|(\beta+1)}$.
%\\
%\\
%\textit{Proof of Theorem \ref{strong gap}.} Fix the strong gap $[\alpha,\beta]$ in $\M$ where $\beta < o(\M)$. Let $\Gamma = \Sigma_1^{\M|\alpha}$. Let
%\begin{eqnarray*}
%\mathcal{C}_\alpha(x,y) &\Leftrightarrow& \exists \gamma < \alpha \ \{y\} \textrm{ is } OD^{\M|\gamma}(x).
%\end{eqnarray*}
%It's easily seen that $\mathcal{C}_\alpha$ is $\Sigma_1^{\M|\alpha}$. Hence $\neg \mathcal{C}_\alpha$ is $\Pi_1^{\M|\alpha}$. We claim that $\neg \mathcal{C}_\alpha$ has no uniformization in $\M|(\beta+1)$. The key to this proof is the following theorem.
%\begin{theorem}
%Suppose $A \in OD^{\M|\beta} \cap \powerset{(\mathbb{R})}$. Then there is a $\Gamma$-suitable premouse $\N$ that locally captures $A$.
%\end{theorem}
%\textbf{Remark:} In fact, more is true. We can take $\N$ in the theorem to be $A$-iterable for normal nondropping trees but we don't need this.
%\\
%\\
%\indent Without loss of generality, suppose $R \in OD^{\M|\beta}(x)$ for some $x\in\mathbb{R}$ is a uniformization of  $\neg \mathcal{C}_\alpha$. Let $y$ be the unique real such that $R(x,y)$. Hence $\{y\} \in OD^{\M|\beta}(x)$ hence is locally captured by a $\Gamma$-suitable premouse $\N$ over $x$. But this implies $y \in \N$ hence $\mathcal{C}_\alpha(x,y)$. Contradiction. This completes the proof of theorem \ref{strong gap}.
%\\
%\\
%\textit{Proof of Theorem \ref{weak gap}.} There are many cases to consider. We only consider one case where $\M$ is active of type II, $\beta = o(\M)$, and $\rho_1(\M) = \mathbb{R}$. Let $F$ be the top extender of $\M$ with critical point $\kappa$ and $\widetilde{\Sigma} = \Sigma^{1,\M}_{\langle G,w_1\rangle}$ be our nonreflecting $\Sigma_1$-type where $G \in ORD^{<\omega}$ and $w_1\in\mathbb{R}$. We may assume $G$ is the Kleene-Brouwer least $H$ such that $\langle H,w_1\rangle$ realizes a nonreflecting $\Sigma_1$-type. Finally, let $\theta = \Theta^\M$. 
%\\
%\indent Let $\beta_0 = \nu(\dot{F}^\M)$ = the sup of generators of $F$. Suppose $\beta_i < \beta$ is defined, let
%\begin{eqnarray*}
%Y_i = \{a \ | \ a \textrm{ is definable over } \M||\beta_i\footnote{$\M||\beta_i$ is just the unique initial segment of the amenable code $\mathfrak{C}_0(\M)$ of $\M$} \textrm{ from}&\textrm{parameters} \\&& \textrm{in } \mathbb{R}^\M\cup\{G,\beta_0,\dots, \beta_{i-1}\} \},
%\end{eqnarray*}
%and
%\begin{equation*}
%\xi_i = \sup (Y_i\cap(\kappa^+)^\M).
%\end{equation*}
%Let $\psi_i$ be the least formula $\psi$ in $\widetilde{\Sigma}$ such that $\M||\beta_i \nvDash \phi[\langle G,w_1\rangle]$. Let $\beta_{i+1}$ be the least $\overline{\beta} > \beta_i$ such that 
%\begin{equation*}
%\M||\overline{\beta} \vDash \psi_i[\langle G,w_1 \rangle] + \dot{F}^{\M||\overline{\beta}} \textrm{ is total on } \powerset{(\kappa)}^{\M|\xi_i} + V = K^\Sigma(\mathbb{R}).
%\end{equation*}
%Because of our specific definition of $\Sigma$-mousehood, the last clause in the above equation should be interpreted as $\M||\overline{\beta}$ is closed under $\Lambda$, where $\Lambda$ is the strategy for $\M_1^{\Sigma,\sharp}$. Recall that the predicate $S$ records a suitable fragment of $\Lambda$ and the statement ``$ V = K^\Sigma(\mathbb{R})$" can be expressed in the language $\mathcal{L}^*$.
%\\
%\indent By the same proof as that of Claim 4.18 in \cite{ScalesK(R)}, we get
%\begin{equation*}
%\M = \bigcup_{i<\omega} Y_i.
%\end{equation*}
%This implies $\sup(\{\beta_i \ | \ i<\omega\}) = \beta$ and $\sup(\{\xi_i \ | \ i<\omega\}) = (\kappa^+)^\M$. Fix uniformly $\Sigma_1^{\M||\beta_i}(G,w_1)$ (in the language $\mathcal{L}$, of course) surjective maps $f_i: \mathbb{R} \twoheadrightarrow Y_i$. For any $x\in \mathbb{R}^\M$ let $\sigma_i^x = 0$ if $f_i(x) \nless_{KB} G$ and = least $\sigma \in \widetilde{\Sigma}$ such that $\M||\beta_i \nvDash \sigma[\langle f_i(x),w_1\rangle]$ otherwise. Let $h_i(x) = 0$ if $f_i(x) \nless_{KB} G$ or $\sigma_i^x$ is $\Sigma_1$ and = least $k \geq i$ such that $\M||\beta_k \vDash \neg\sigma^x_i[\langle f_i(x),w_1\rangle]$ otherwise. Then for some $w_2\in\mathbb{R}^\M$, uniformly in $i$, the functions $h_i, x\mapsto \sigma^x_i$ are $\Sigma_2^{\M|\beta_i}(G,w_1,w_2)$. This uses the coding lemma applied to sets in $\M|\theta$, $\beta_i>\theta$, and the fact that the transitive collapses of the $Y_i$ are in $\M|\theta$.
%\\
%\indent Now let $\mathcal{L}^{**}$ be an extension of $\mathcal{L}$ that describes $\M$ as the union of the $Y_i$. $\mathcal{L}^{**}$ consists of the extra constant symbols $\{\dot{w_1},\dot{w_2},\dot{G},(\dot{\M_k},\dot{\beta_k} \ | \ k<\omega)\}$. Let $B_0$ be the set of $\Sigma_0$ formulae in $\mathcal{L}^{**}$. Let 
%\begin{equation*}
%S_0 = \{\phi \in B_0 \ | \ \phi \textrm{ is a sentence and } \M\vDash \phi\}.
%\end{equation*}
%We say a formula $\phi \in B_0$ has support $m$ if it can only refer to $\{\dot{w_1},\dot{w_2},\dot{G},(\dot{\M_k},\dot{\beta_k} \ | \ k<m)\}$. Let
%\begin{equation*}
%S_m = \{\langle\phi,x_1,\dots,x_k\rangle \ | \ \phi\in B_0 \textrm{ has support } m \wedge \M\vDash \phi[x_1,\dots,x_k]\}.
%\end{equation*}
%Note that $\forall i\exists \gamma < \beta \ S_i$ is $OD^{\M|\gamma}(w_1,w_2)$. Once we isolate the $S_i$. We can proceed as in \cite{Scalesweakgap} to get the desirable scale.



==> Setup.tex <==
\section{BASIC SETUP}

Working in $\sf{ZF} + \sf{DC}$, suppose $\omega_1$ is $\powerset(\mathbb{R})$-strongly compact as witnessed by $\mu$. We assume $V = L(\powerset(\mathbb{R}),\mu)$.\footnote{$V$ is a structure of the language of set theory with an extra predicate for $\mu$.} For each $\sigma \in \powerset_{\omega_1}(\powerset(\mathbb{R}))$, let $\mmM_\sigma = \rm{HOD}^{(V,\mu)}_{\sigma\cup \{\sigma\}}$. For $\sigma \in \powerset_{\omega_1}(\powerset(\mathbb{R}))$ and $x\in \sigma$, let $\mmH_{x,\sigma} = \rm{HOD}_{\{x,\sigma\}}^{(V,\mu)}$. Let $\mmM = \prod_{\sigma} \mmM_\sigma\slash \mu$. Let $\mmH_x = \prod_{\sigma} \mmH_{x,\sigma} \slash \mu$ for each $x\in \powerset(\mathbb{R})$; note that $\forall^*_\mu \sigma \ x\in \sigma$ by fineness of $\mu$. We note that by $\sf{DC}$ and countable completeness of the measure $\mu$, the ultraproducts are well-founded (we identify them with their transitive collapse). The following lemma concerns Los theorem for $\mu$-ultraproducts.

\begin{lemma}
\label{Los}
\begin{enumerate}
\item Let $x\in \powerset(\mathbb{R}))$. Let $\varphi(v_0,v_1)$ be a formula in the language of set theory (augmented by a predicate for $\mu$) and $[f]_\mu\in H_x$. Then $\exists x (\mmH_x \vDash \varphi[x,[f]_\mu])$ if and only if $\forall^*_\mu \sigma \ \exists x (\mmH_{x,\sigma} \vDash \varphi[x,f(\sigma)])$. Consequently, the ultraproduct satisfies Los theorem. 
\item Suppose $\mu$ is also normal. Let $\psi(v_0,v_1)$ be a formula in the language of set theory (augmented by a predicate for $\mu$) and $[f]_{\mu}\in M$. Then $\exists x \ (\mmM\vDash \psi[x,[f]_{\mu}])$ if and only if $\forall^*_{\mu}\sigma \ \exists x \ (\mmM_\sigma\vDash \psi[x,f(\sigma)])$. Consequently, the ultraproduct satisfies Los theorem.
\end{enumerate}
\end{lemma} 
\begin{proof}
(1) holds since each $\mmH_{x,\sigma}$ has an $OD_{\{x,\sigma\}}$-wellordering, uniformly in $\sigma$. The usual proof of Los theorem goes through with this observation.

We prove (2) by induction on the complexity of the formula $\psi$. It's enough to show that if $\forall^*_{\mu}\sigma \ \exists x \ (\mmM_\sigma\vDash \psi[x,f(\sigma)])$ then $\exists x \ (\mmM\vDash \psi[x,[f]_{\mu}])$. For a typical $\sigma$, let $A_\sigma = \{x \in \sigma \ | \ \exists y\in OD(x) \ (\mmM_\sigma \vDash \psi[y,f(\sigma)])\}$. By our hypothesis, the function $F(\sigma) = A_\sigma$ is such that $\forall^*_\mu \sigma \ (F(\sigma)\neq \emptyset \wedge F(\sigma)\subseteq \sigma)$. By normality of $\mu$, there is an $x$ such that $\forall^*_\mu \sigma (x\in F(\sigma))$. Fix such an $x$ and let $g(\sigma)$ be the least OD$(x)$ set $y$ such that $\mmM_\sigma \vDash \psi[y,f(\sigma)]$ if such a $y$ exists and $\emptyset$ otherwise. Then $\mmM \vDash \psi[[g]_\mu, [f]_\mu]$. 
\end{proof}

Let $[\sigma\mapsto \omega_1^\sigma]_\mu = \omega_1$ and $[\sigma\mapsto\Theta^\sigma]_\mu = \Theta$. $\mu$ induces a countably complete measure $\nu$ on $\kappa =_{\rm{def}} \omega^V_1$. 

\begin{proposition}\label{ACFails}
\begin{enumerate}
\item $\kappa$ is measurable in both $\mmM_\sigma$ and $\mmH_{x,\sigma}$ for all $\sigma$ and for all $x\in \sigma$.
\item $\sf{AC}$ fails; in fact, there cannot be an $\omega_1$-sequence of distinct reals.
\end{enumerate}
\end{proposition}
\begin{proof}
(1) is immediate. For (2), suppose $\langle x_\alpha \ | \ \alpha<\kappa \rangle$ is an $\kappa$-sequence of distinct reals. By countable completeness of $\nu$, for each $n<\omega$, there is a $k_n<\omega$ such that 
\begin{center}
$\forall^*_\nu \alpha \ x_\alpha(n) = k_n$.
\end{center} 
Let $x = \langle k_n \ | \ n<\omega \rangle$. By countable completeness again, 
\begin{center}
$\forall^*_\nu \alpha \ x_\alpha = x$.
\end{center}
Contradiction.
\end{proof}
Fix $x,\sigma$; it is easy to see that, letting $H = \mmH_{x,\sigma}$, then the usual Vopenka argument, using Proposition \ref{ACFails}, shows that if $A$ is a bounded subset of $\kappa$, then there is a forcing $\mathbb{P}\in \mmH_{x,\sigma}$ of size smaller than $\kappa$ such that there is a $\mmH_{x,\sigma}$-generic $G_A\subseteq \mathbb{P}$ such that $\mmH_{x,\sigma}[G_A]= \mmH_{x,\sigma}[A]$. 

Let $\Xi = [\sigma\mapsto \kappa]_\mu$.
\begin{lemma}
\label{propertiesofM}
\begin{enumerate}
\item Suppose $A\subseteq \mathbb{R}$, then $A=[\sigma\mapsto A\cap \sigma]_\mu$. Consequently, $\powerset(\mathbb{R})\subseteq\mmM$. 
\item $\Xi \geq \Theta$ and $\Xi$ is measurable in $\mmH_x$ for all $x\subseteq \mathbb{R}$. If in addition, $\mu$ is normal, then $\Xi > \Theta$ and is measurable in $\mmM$.
\end{enumerate}
\end{lemma}
\begin{proof}
For each $\sigma\in \powerset_{\omega_1}(\powerset(\mathbb{R}))$, let $\mathbb{R}_\sigma = \mathbb{R}\cap \sigma$. To prove (1), first note that for any $x\in\mathbb{R}$, $x = [\sigma\mapsto x]_\mu$; this uses countable completeness of $\mu$ and is similar to the argument in Proposition \ref{ACFails}. Let $A\subseteq \mathbb{R}$. By fineness of $\mu$, $\forall^*_\mu \sigma \ (A\in \sigma)$. This means $\forall^*_{\mu}\sigma \ (A\cap \mathbb{R}_\sigma \in \mathscr{M}_\sigma)$ and $A = [\sigma\mapsto A\cap \sigma] \in \mmM$ (by Lemma \ref{Los}). This finishes the proof of (1). 
\\
\indent For (2), recall that $\powerset(\mathbb{R})\subseteq \mmM$. Let $\leq$ be a prewellordering of $\mathbb{R}$ in $\mmM$ of length $\alpha$. For each $\sigma$, let $\alpha_\sigma$ be the length of $\leq \cap \mathbb{R}_\sigma$. Then $\alpha = [\sigma\mapsto \alpha_\sigma]_\mu$. Note that we have enough instances of Los theorem to conclude this (and don't need normality of $\mu$). $\forall^*_\mu \ \alpha_\sigma < \kappa$ since $\mathbb{R}_\sigma$ is countable; this gives $\alpha < \Xi$. The fact that $\Xi$ is measurable in $\mmH_x$ follows from Proposition \ref{ACFails} (1) and Lemma \ref{Los} (1).

Suppose $\mu$ is also normal. Then $\forall^*_\mu \sigma \ \mathbb{R}_\sigma=\mathbb{R}^{\mathscr{M}_\sigma}$ and by Lemma \ref{Los} (2), $\Theta=[\sigma\mapsto \Theta^{\mathscr{M}_\sigma}]_\mu$ and by Proposition \ref{ACFails} and the fact that $\mathbb{R}_\sigma$ is countable, $\powerset(\mathbb{R}_\sigma)^{\mmM_\sigma}$ is countable, hence $\Theta^\sigma<\kappa$. This means $\Xi>\Theta$. Again, by Proposition \ref{ACFails} and Proposition \ref{Los} (2) $\Xi$ is measurable in $\mmM$.
\end{proof}

Suppose $N$ is a transitive structure of a sufficiently fragment of $\sf{ZF} + \sf{DC}$ and there is a surjection $\pi: \powerset(\mathbb{R})\rightarrow N$. We then let $\mu_N$ be the measure on $\powerset_{\omega_1}(N)$ defined from $\mu$ as in Lemma \ref{factsaboutnfm} (the measure depends on $\pi$ also but we don't need to keep track of the surjection).
%We then observe that $\Omega$ is measurable in $M$ and in $H$. This is because $\omega_1$ is measurable in $M_\sigma$ and $H_\sigma$ for all $\sigma$. Using the fact that there are no sequences of $\omega_1^V$ distinct reals and Lemma \ref{Los}, we get, by a standard Vopenka argument, for any $A\in M$ such that $A$ is a bounded subset of $\Omega$, there is an $H$-generic $G_A$ (for a forcing of size smaller than $\Omega$) such that $A \in H[G_A] \subseteq M$ and $\Omega$ is also measurable in $H[G_A]$.

